The Coupled Rejection Sampler

We propose a coupled rejection-sampling method for sampling from couplings of arbitrary distributions. The method relies on accepting or rejecting coupled samples coming from dominating marginals. Contrary to existing acceptance-rejection coupling methods, the variance of the execution time of the proposed method is limited and stays finite as the two target marginals approach each other in the sense of the total variation norm. In the important special case of coupling multivariate Gaussians with different means and covariances, we derive positive lower bounds for the resulting coupling probability of our algorithm, and we then show how the coupling method can be optimized in closed form. Finally, we show how we can modify the coupled rejection-sampling method to propose from coupled ensemble of proposals, so as to asymptotically recover a maximal coupling. We then apply the method to the problem of coupling rare events samplers, derive a parallel coupled resampling algorithm to use in particle filtering, and show how the coupled rejection-sampler can be used to speed up unbiased MCMC methods based on couplings.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> successful_coupling_tikz.tex <==
\begin{tikzpicture}
\tikzset{node distance=3.5cm, %
         every state/.style={ %
           minimum size=2.4cm,
           semithick,
           fill=gray!10},
         initial text={},     %
         double distance=4pt, %
         every edge/.style={  %
         draw,
           ->,>=stealth',     %
           auto,
           thick}}
\node[state] (s1) {Initial State};
\node[state, above right of=s1] (s2) {$\hat{X} \neq \hat{Y}$};
\node[state, below right of=s1] (s3) {$\hat{X} = \hat{Y}$};

\node[state, above right of=s2] (s21) {$A_X=A_Y=0$};
\node[state, right of=s2]       (s22) {$A_X=A_Y=1$};
\node[state, below right of=s2] (s23) {$A_X \neq A_Y$};

\node[state, below right of=s3] (s31) {$A_X=A_Y=0$};
\node[state, right of=s3]       (s32) {$A_X=A_Y=1$};

\node[state, right of=s22] (s4) {Unsuccessful};
\node[state, right of=s32] (s5) {  Successful};


\draw (s1) edge[bend right]     (s2);
\draw (s1) edge[bend left]      (s3);

\draw (s2) edge[bend right]     (s21);
\draw (s2) edge                 (s22);
\draw (s2) edge[bend left]      (s23);

\draw (s3) edge[bend right]     (s23);
\draw (s3) edge                 (s32);
\draw (s3) edge[bend left]      (s31);

\draw (s21) edge[bend right]    (s1);
\draw (s31) edge[bend left]     (s1);

\draw (s23) edge[bend right]    (s4);
\draw (s22) edge                (s4);

\draw (s32) edge                (s5);

\end{tikzpicture}

